Generation and effects of primordial magnetic fields during inflation

In this thesis, we aim to investigate the mechanisms underlying the genesis of magnetic fields in the Universe and explore their potential in addressing the matter-antimatter asymmetry. We construct consistent models that generate the helical magnetic field consistent with observations. We also develop an effective field theory approach to magnetogenesis, where the choice of EFT parameters describes the magnetogenesis scenario in the early Universe, and different choices of parameters correspond to different models. Our EFT explicitly shows that generating primordial magnetic fields requires two necessary conditions: conformal invariance breaking and causal propagation. Furthermore, we establish that the presence of a strong magnetic field near compact objects, such as neutron stars, aids in understanding the phenomenon of Fast radio bursts through the conversion of gravitational waves to electromagnetic waves in the background of a strong transverse magnetic field.

==> format.tex <==
\usepackage{graphicx,epstopdf}
\usepackage{a4wide}
\usepackage{fancyhdr}
%\usepackage{pdfpages}
\usepackage[dvips]{epsfig}
\usepackage{palatino,amsmath,float,multicol,shadow,fancybox,amsfonts,amsthm}
%\usepackage{chapterbib}
\usepackage{bm}% bold math
\usepackage{float}
\usepackage{cite}
\usepackage{gensymb}
\usepackage{array}
%\usepackage[number]{natbib}
%\usepackage{notoccite}
%\usepackage[number,sort&compress]{natbib}
\usepackage{amssymb}
\usepackage{stmaryrd}
\usepackage{mathrsfs}
\usepackage{amsmath}
%\usepackage[utf8]{inputenc}
\usepackage[nottoc]{tocbibind}
\usepackage{makeidx}
\usepackage{relsize}
%\usepackage[T1]{fontenc}
%\usepackage[bitstream-charter]{mathdesign}
%\usepackage{charter}
\usepackage[sc]{mathpazo}
\usepackage{subcaption}
\usepackage{tabu}
\usepackage{longtable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{chngcntr}
\usepackage[normalem]{ulem}
%\bibliography{refs}
\usepackage{url}
%\usepackage{subcaption}
\usepackage[titletoc]{appendix}
\usepackage{enumitem}
\usepackage{hhline}
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{graphics}
%\usepackage[titletoc]{}
\usepackage[colorlinks]{hyperref}
\usepackage{multirow}
\usepackage{caption}
%\usepackage{subfig}
\usepackage[titles]{tocloft}
\usepackage[normalem]{ulem}
\usepackage{rotating}
%\usepackage[caption=false]{subfig}
%\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{caption}
%\usepackage{subcaption}
\usepackage{amsthm,url}
%\usepackage{color}
%\usepackage{color,ulem}
\usepackage[dvipsnames]{xcolor}
\pagestyle{fancy}
\setlength{\headheight}{15pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\chapquote}[3]{\begin{quotation} \textit{#1} \end{quotation} \begin{flushright} - #2, \textit{#3}\end{flushright} }
\newcommand{\upchi}{\protect\raisebox{2.5pt}{$\chi$}}
\renewcommand{\headrulewidth}{.1pt}
\fancyhead[LE,RO]{{\thepage}}
\fancyhead[RE]{\nouppercase{{\leftmark}}}
\fancyhead[LO]{\nouppercase{{\rightmark}}} \fancyfoot{}
\def\baselinestretch{1.1}
%\usepackage{here}
%\usepackage{newcent}
\pagenumbering{roman}
\date{October 6, 2023}
\clubpenalty=10000 \widowpenalty=10000

% The \singlespace macro switches to single spaced lines
%\newcommand{\singlespace}{\par\renewcommand{\baselinestretch}{1}\small\normalsize\par}
%\newcommand{\doublespace}{\par\renewcommand{\baselinestretch}{1.5}\small\normalsize\par}
%-----------------------------------------------------------------------------
\newcommand{\note}{\color{black}}
% THEOREM Environments ---------------------------------------------------
%\setlength{\textheight}{19.5 cm} \setlength{\textwidth}{12.5 cm}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{hypothesis}[theorem]{Hypothesis}
%\newenvironment{proof}{\paragraph{Proof:}}{\hfill$\square$}
\renewcommand{\theequation}{\arabic{chapter}.\arabic{equation}}
\newcommand{\mainidx}[1]{{\it #1}}
  \newcommand{\boldidx}[1]{{\bf #1}}
\hypersetup{
    %bookmarks=false,         % show bookmarks bar?
    %pdfstartview={FitH},    % fits the width of the page to the window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=blue,          % color of internal links
    citecolor=red,        % color of links to bibliography
    urlcolor=magenta
    %filecolor=blue,      % color of file links
    %urlcolor=blue           % color of external links
}
%\hypersetup{
%    %bookmarks=true,        % show bookmarks bar?
%    unicode=false,          % non-Latin characters in Acrobat�s bookmarks
%    pdftoolbar=true,        % show Acrobat�s toolbar?
%    pdfmenubar=true,        % show Acrobat�s menu?
%    pdffitwindow=false,     % window fit to page when opened
%    pdfstartview={FitH},    % fits the width of the page to the window
%    pdftitle={My title},    % title
%    pdfauthor={Author},     % author
%    pdfsubject={Subject},   % subject of the document
%    pdfcreator={Creator},   % creator of the document
%    pdfproducer={Producer}, % producer of the document
%    pdfkeywords={keywords}, % list of keywords
%    pdfnewwindow=true,      % links in new window
%   
%    filecolor=violet,      % color of file links
%    
%     %bookmarks=false,         % show bookmarks bar?
%    %pdfstartview={FitH},    % fits the width of the page to the window
%    colorlinks=true,       % false: boxed links; true: colored links
%    linkcolor=red,          % color of internal links
%    citecolor=blue,        % color of links to bibliography
%    urlcolor=magenta
%    %filecolor=blue,      % color of file links
%    %urlcolor=blue           % color of external links}

%---------------------------------------------------------------------------
\newcommand {\apgt} {\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand {\aplt} {\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }

\makeatletter
\def\myfnt{\ifx\protect\@typeset@protect\expandafter\footnote\else\expandafter\@gobble\fi}
\makeatother

\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\newcommand{\comm}[1]{}


\usepackage{etoolbox}

\AtBeginEnvironment{subappendices}{%
	\chapter*{Appendix}
	\addcontentsline{toc}{chapter}{Appendices}
	\counterwithin{figure}{section}
	\counterwithin{table}{section}
}
	

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bn{\begin{enumerate}}
\def\en{\end{enumerate}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}

\def\etc{\textit{etc. }}
\def\eg{\textit{eg, }}
\def\lt{\left}
\def\ll{\left}
\def\rt{\right}
\def\rr{\right}
\def\nn{\nonumber}
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcp{\textcolor{purple}}

\def\c{\times}
\def\mc{\mathcal}
\def\mb{\mathbf}

\def\Hs{\mathcal{H}_{s}}
\def\paramVec{\bar{\theta}}
\def\bestEst{\bar{\theta}_{best}}
\def\trueParam{\bar{\theta}_{true}}

\def\h{{h}}
\def\th{\tilde{\mb{h}}}
\def\tf{\tilde{\mb{f}}}
\def\Ro{\boldsymbol{\rho}}
\def\Hz{\text{~Hz}}
\def\Mpc{\text{~Mpc}}
\def\Msn{M_\odot}
\def\crossI{\mathcal{I}}

\def\snf{{S_n}(f)}
\def\hI{\h^I}
\def\hf{\tilde{\h}}
\def\hfp{\tilde{\h}_{+}}
\def\hfpI{\hfp^I}
\def\hfc{\tilde{\h}_{\times}}
\def\hfcI{\hfc^I}
\def\hp{\h_{+}}
\def\hc{\h_{\times}}
\def\hpI{\hp^I}
\def\hcI{\hc^I}
\def\hzero{\hf_0}
\def\hzeroStar{\hzero^*}

\def\diota{\Delta\iota}
\def\dcosIota{\Delta\cosIota}

% antenna pattern
\def\F{\mb{F}}
\def\FI{{\F}^I}
\def\Fp{\mb{F_{+}}}
\def\FpI{\mb{F}^I_{+}}
\def\Fc{\mb{F_{\times}}}
\def\FcI{\mb{F}^I_{\times}}
\def\FImodSq{|\FI|^2}
\def\FpImodSq{|\FpI|^2}
\def\FcImodSq{|\FcI|^2}
\def\FpInormSq{\|\FpI\|^2}
\def\FcInormSq{\|\FcI\|^2}
\def\FnormSq{\|\F\|^2}
\def\Fex{\mathcal{F}}
\def\FexI{{\Fex^I}}
\DeclareMathOperator*{\argmax}{argmax}
\def\FexIstar{{\Fex^I}^*}
\def\dFexdpsi{\frac{\partial\Fex}{\partial\psi}} 
\def\dFexdCosIota{\frac{\partial\Fex}{\partial\cos\iota}} 
\def\dFexdthetaP{\frac{\partial\Fex}{\dtheta^p}} 
\def\dFexdthetaq{\frac{\partial\Fex}{\dtheta^q}} 

\def\hfmodSq{|\hf_0|^2}
\def\dtheta{\partial\theta}
\def\dhf{\partial\tilde{\h}}
\def\tp{\mb{t_{+}}}
\def\tm{\mb{t_{-}}}
\def\dI{\mb{d}^I}
\def\dIstar{{\mb{d}^I}^*}
\def\dl{\mb{d_L}}
\def\lndl{\ln{\dl}}
\def\Mc{\mc{M}}
\def\intsnropt{\int_{0}^{\infty}\frac{\vert\hf_0\vert^2}{S_n(f)}df}
\def\squaredFex{\|\Fex\|^2}
\def\integral{\int_{0}^{\infty}}
\def\dtaudalpha{\frac{\partial\tau^I}{\partial\theta^\alpha}}
\def\snrsqSingle{\Ro_{s}^2}
\def\snrsqNet{\Ro_{net}^2}
\def\sumI{\sum_{I}}
\def\cosIota{\cos{\iota}}
\def\cosSqIota{\cos^2\iota}
\def\onePlusCosSqIota{1+\cos^2\iota}
\def\onePlusCosSqIotaBy2{\frac{\onePlusCosSqIota}{2}}

\def\lalinference{\textit{LALInference }}
\def\delPsiByDelMc{\frac{\partial\Psi}{\partial\Mc}}
\def\delPsiByDelEta{\frac{\partial\Psi}{\partial\eta}}

\def\hsFiveMM{\hspace{5mm}}
\def\hsThreeMM{\hspace{3mm}}
\def\hsOneCM{\hspace{1cm}}

\def\lat{\mb{\tiny{Lat}}}
\def\lon{\mb{\tiny{Long}}}
\def\latI{\lat^I}
\def\lonI{\lon^I}
%-----------------------
\def\tmax{$t_{max}$}
\def\Eiso{E_{iso}}
\def\tv{\theta_v}
\def\tj{\theta_j}
\def\tp{t_{\rm peak}}
\def\ts{t_{\rm start}}
\def\tvj{\theta_{vj}}
\def\eB{\epsilon_B}
\def\eE{\epsilon_E}
\def\p{p}
\def\Msun{M_\odot}
\def\msm{\mathsmaller}
\def\tc{\textcolor{red}}
\def\tcg{\textcolor{green}}
\def\tcb{\textcolor{blue}}
\def\dg{^\circ}
%\newcommand{\blue}{\color{blue}}
%\newcommand{\red}{\color{red}}

 \def\rAG{\mathbf{r_{\mathsmaller {AG,BNS}}}}
 \def\RAG{\mathbf{R_{\mathsmaller {AG,BNS}}}}
 \def\Vdet{\mathbf{V_{\mathsmaller {det}}}}
 \def\fgwdet{\mathbf{f_{\mathsmaller {GWdet}}}}
 \def\fagdet{\mathbf{f_{\mathsmaller {AGdet}}}}
 \def\rBNS{\mathbf{r_{\mathsmaller{BNS}}}}
 

\def\wrt{\textit{w.r.t }}
\def\thatis{\textit{ie, }}

\def\phiOrb{\phi_{orb}}

\def\devP{$\delta \hat{p}_i$}
\def\devPhi{$\delta \hat{\varphi}_i$}
\def\devPhiL{$\delta \hat{\varphi}_{il}$}
\def\devBeta{$\delta \hat{\beta}_i$}
\def\devAlpha{$\delta \hat{\alpha}_i$}

\newcommand*{\red}{\textcolor{red}}%new macro for text colour
\newcommand*{\blue}{\textcolor{blue}}
\newcommand*{\green}{\textcolor{green}}
\def\rh{\curvearrowright}
\def\lh{\curvearrowleft}
%\def\tc{\textcolor{red}}
\def\tcg{\textcolor{green}}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\newcommand{\hslashslash}{%
	\raisebox{.3ex}{%
		\scalebox{.9}{%
			\rotatebox[origin=c]{25}{$-$}%
		}%
	}%
}
\newcommand{\Islash}{%
	{%
		\vphantom{d}%
		\ooalign{\kern-.25em\smash{\hslashslash}\hidewidth\cr$I$\cr}%
		\kern.05em
	}%
}


